Task-Based Tensor Computations on Modern GPUs

Domain-specific, fixed-function units are becoming increasingly common in modern processors. As the computational demands of applications evolve, the capabilities and programming interfaces of these fixed-function units continue to change. NVIDIA's Hopper GPU architecture contains multiple fixed-function units per compute unit, including an asynchronous data movement unit (TMA) and an asynchronous matrix multiplication unit (Tensor Core). Efficiently utilizing these units requires a fundamentally different programming style than previous architectures; programmers must now develop warp-specialized kernels that orchestrate producer-consumer pipelines between the asynchronous units. To manage the complexity of programming these new architectures, we introduce Cypress, a task-based programming model with sequential semantics. Cypress programs are a set of designated functions called \emph{tasks} that operate on \emph{tensors} and are free of communication and synchronization. Cypress programs are bound to the target machine through a \emph{mapping} specification that describes where tasks should run and in which memories tensors should be materialized. We present a compiler architecture that lowers Cypress programs into CUDA programs that perform competitively with expert-written codes. Cypress achieves 0.88x-1.06x the performance of cuBLAS on GEMM, and between 0.80x-0.98x the performance of the currently best-known Flash Attention implementation while eliminating all aspects of explicit data movement and asynchronous computation from application code.

==> axpby.tex <==
\begin{figure}
\begin{subfigure}[h]{0.59\textwidth}
\begin{lstlisting}
@task("axpby", Inner, reads["x","y"], writes=["y"])
def axpby_host(x: tensor[1,f32],
               y: tensor[1,f32],
               a: f32, b: f32):
  # Tunable parameters are specified in the mapping.
  THREADS = tunable(int)
  # Break the problem into an element per thread.
  N = x.shape[0]
  xp = partition_by_blocks(x, (THREADS,))
  yp = partition_by_blocks(y, (THREADS,))
  for i in prange(cdiv(N, THREADS)):
    launch("axpby", xp[i], yp[i], a, b)

@task("axpby", Inner, reads["x","y"], writes=["y"])
def axpby_inner(x: tensor[1,f32],
                y: tensor[1,f32],
                a: f32, b: f32):
  PROCS, TILE = tunable(int), tunable(int)
  N = x.shape[0]
  xp = partition_by_blocks(x, (TILE,))
  yp = partition_by_blocks(y, (TILE,))
  for i in prange(PROCS):
    launch("axpby", xp[i], yp[i], a, b)
    
@task("axpby", Leaf, reads["x","y"], writes=["y"])
def axpby_thread(x: tensor[1,f32],
                 y: tensor[1,f32],
                 a: f32, b: f32):
  y[0] = a * x[0] + b * y[0]
\end{lstlisting}
\caption{Logical program description.}
\label{fig:cypress-axpby-tasks}
\end{subfigure}\hfill%
\begin{subfigure}[h]{0.40\textwidth}
\begin{lstlisting}
[
  TaskMapping(
    instance="axpby_host",
    variant="axpby_host",
    proc=HOST,
    mems=[GLOBAL, GLOBAL],
    tunables={"THREADS": 128},
    entrypoint=True,
    calls=["axpby_block"]
  ),
  TaskMapping(
    instance="axpby_block",
    variant="axpby_inner",
    proc=BLOCK,
    mems=[GLOBAL, GLOBAL],
    tunables={"PROCS": 4, "TILE": 32},
    calls=["axpby_warp"]
  ),
  TaskMapping(
    instance="axpby_warp",
    variant="axpby_inner",
    proc=WARP,
    mems=[GLOBAL, GLOBAL],
    tunables={"PROCS": 32, "TILE": 1},
    calls=["axpby_thread"]
  ),
  TaskMapping(
    instance="axpby_thread",
    variant="axpby_thread",
    proc=THREAD,
    mems=[GLOBAL, GLOBAL]
  )
]
\end{lstlisting}
\caption{Mapping specification.}
\label{fig:cypress-axpby-mapping}
\end{subfigure}
\caption{Na\"ive AXPBY ($y = \alpha \cdot x + \beta \cdot y$) in \name{}.}
\end{figure}

==> dep-analysis-alg.tex <==
\begin{algorithm}[t]
\caption{Non-overlapping repeated sub-strings.}
\label{fig:repeats-algorithm}
\footnotesize
\SetKwProg{DepAnalysis}{DepAnalysis}{}{}

\SetKwFunction{FSuffixArray}{SuffixArray}
\SetKwFunction{FSort}{Sort}
\SetKwFunction{FDeduplicate}{Deduplicate}
\SetAlgoLined
\DontPrintSemicolon

\DepAnalysis{$(T)$}{
    \ForEach{$s \in T$}{
        
    }
    $SA, LCP \gets$ \FSuffixArray{$S$} \;
    \tcc{Candidates are tuples of string length, the repeated sub-string, and starting position.}
    $C \gets []$\;
    \ForEach{$i \in [0, |SA| - 1)$}{
        \tcc{Extract adjacent suffix array entries and their overlap length.}
        $s1, s2, p \gets SA[i], SA[i+1], LCP[i]$ \;
        \If{$[s1:s1+p) \cap [s2:s2+p) = \emptyset$}{
            \tcc{$S[s1:s1+p]$ and $S[s2:s2+p]$ are repeated strings that do not overlap in $S$, so they are candidates.}
            $r \gets S[s1:s1+p]$ \;
            $C \gets C + [(p, r, s1), (p, r, s2)]$ \;
        }
        \Else{
            \tcc{$S[s1:s1+p]$ and $S[s2:s2+p]$ overlap in $S$. Assume $s2 > s1$, the other case is symmetric. In this case, the overlap is a collection of repeats of $S[s1:s1+d]$, by the structure of the suffix array.}
            $d \gets s2 - s1$\;
            \tcc{Break prefix into two chunks of repeated pieces of $S[s1:s1+d]$.}
            $l \gets (p + d) / 2$ \;
            \tcc{Remove trailing tokens.}
            $l \gets l - (l \% d)$\;
            $r \gets S[s1:s1+l]$ \;
            $C \gets C + [(l, r, s1), (l, r, s1 + l)]$\;
        }
    }
    \tcc{Sort the candidates by decreasing length and by increasing sub-string and start position.}
    \FSort{$C$}\;
    \tcc{Greedily collect sub-strings that do not overlap with previously chosen sub-strings.}
    $I, R \gets [], []$ \;
    \ForEach{$(l, \_, s) \in C$} {
        \If{$[s, s+l)$ \text{does not intersect} $I$}{
            $I \gets I + [[s, s+l)]$\;
            $R \gets R + [S[s:s+l]]$\;
        }
    }
    \Return{$R$}
}
\end{algorithm}

==> r1upd.tex <==
\begin{figure}
\begin{subfigure}[h]{0.62\textwidth}
\begin{lstlisting}
@task("r1upd", Inner, reads["A","x","y"], writes=["A"])
def r1upd_host(A: tensor[2,f32],
               x: tensor[1,f32],
               y: tensor[1,f32]):
  # Tunable parameters are specified in the mapping.
  B = tunable(int), tunable(int)
  N = A.shape[0]
  # Break the problem into BxB tiles.
  Ap = partition_by_blocks(A, (B, B))
  xp = partition_by_blocks(x, (B,))
  yp = partition_by_blocks(y, (B,))
  for i, j in prange(cdiv(N, B), cdiv(N, B)):
    launch("r1upd", Ap[i, j], xp[i], yp[j])

@task("r1upd", Inner, reads["A","x","y"], writes=["A"])
def r1upd_block(A: tensor[2,f32],
                x: tensor[1,f32],
                y: tensor[1,f32]):
  # Break up the rows amongst the warps.
  WARPS = tunable(int)
  N = A.shape[0]
  Ap = partition_by_blocks(A, (N/WARPS, N))
  for i in prange(WARPS):
    launch("r1upd", Ap[i], x, y)

@task("r1upd", Inner, reads["A","x","y"], writes=["A"])
def r1upd_warp(A: tensor[2,f32],
               x: tensor[1,f32],
               y: tensor[1,f32]):
  THREADS = tunable(int)
  N, M = A.shape[0], A.shape[1]
  Ap = partition_by_blocks(A, (1, THREADS))
  yp = partition_by_blocks(y, (1,))
  for i, j in srange(N, M/THREADS):
    launch("r1upd", Ap[i, j], x, yp[i])

@task("r1upd", Inner, reads["A","x","y"], writes=["A"])
def r1upd_inner(A: tensor[2,f32],
                x: tensor[1,f32],
                y: tensor[1,f32]):
  THREADS = tunable(int)
  N, M = A.shape[0], A.shape[1]
  Ap = partition_by_blocks(A, (1, 1))
  xp = partition_by_blocks(x, (1,))
  for i in prange(THREADS):
    launch("r1upd", Ap[0, i], x[i], y)

@task("r1upd", Inner, reads["A","x","y"], writes=["A"])
def r1upd_thread(A: tensor[2,f32],
                 x: tensor[1,f32],
                 y: tensor[1,f32]):
  # Written in CUDA C++.
  A[0, 0] = x[0] * y[0]
\end{lstlisting}
\caption{Logical program description.}
\label{fig:cypress-gemm-tasks}
\end{subfigure}\hfill%
\begin{subfigure}[h]{0.37\textwidth}
% \begin{lstlisting}
% [
%   TaskMapping(
%     instance="gemm_host",
%     variant="gemm_host",
%     proc=HOST,
%     mems=[GLOBAL, GLOBAL, GLOBAL],
%     tunables={"U": 256, "V": 256},
%     entrypoint=True,
%     calls=["gemm_block"]
%   ),
%   TaskMapping(
%     instance="gemm_block",
%     variant="gemm_block",
%     proc=BLOCK,
%     mems=[GLOBAL, GLOBAL, GLOBAL],
%     tunables={"W": 64},
%     calls=["fill_tile",
%            "gemm_tile",
%            "copy_tile"],
%     warpspecialize=True,
%     pipeline=3
%   ),
%   TaskMapping(
%     instance="gemm_tile",
%     variant="gemm_tile",
%     proc=BLOCK,
%     mems=[NONE, SHARED, SHARED],(*\label{fig:cypressmapping:nonemap}*)
%     tunables={"WGS": 2},
%     calls=["gemm_warpgroup"]
%   ),
%   TaskMapping(
%     instance="gemm_warpgroup",
%     variant="gemm_inner",
%     proc=WARPGROUP,
%     mems=[NONE, SHARED, SHARED],
%     tunables={"PIECES": 4,
%               "PROC": WARP}
%     calls=["gemm_warp"]
%   ),
%   TaskMapping(
%     instance="gemm_warp",
%     variant="gemm_inner",
%     proc=WARP,
%     mems=[NONE, SHARED, SHARED],
%     tunables={"PIECES": 32,
%               "PROC": THREAD}
%     calls=["gemm_thread"]
%   ),
%   TaskMapping(
%     instance="gemm_thread",
%     variant="gemm_thread",
%     proc=THREAD,
%     mems=[REGISTER, SHARED, SHARED],
%   ),
%   # Mappings for `fill` and
%   # `copy` task trees elided.
% ]
% \end{lstlisting}
\caption{Mapping specification.}
\label{fig:cypress-gemm-mapping}
\end{subfigure}
\end{figure}
